Why do Larger Models Generalize Better? A Theoretical Perspective via the XOR Problem

Empirical evidence suggests that neural networks with ReLU activations generalize better with over-parameterization. However, there is currently no theoretical analysis that explains this observation. In this work, we provide theoretical and empirical evidence that, in certain cases, overparameterized convolutional networks generalize better than small networks because of an interplay between weight clustering and feature exploration at initialization. We demonstrate this theoretically for a 3-layer convolutional neural network with max-pooling, in a novel setting which extends the XOR problem. We show that this interplay implies that with overparamterization, gradient descent converges to global minima with better generalization performance compared to global minima of small networks. Empirically, we demonstrate these phenomena for a 3-layer convolutional neural network in the MNIST task.

==> proofs.tex <==
\section{Proof Sketch and Insights}
\label{sec:proofs}
In this section we sketch the proof of Theorem \ref{thm:generalization_gap}. The theorem follows  from two theorems: Theorem \ref{thm:main} for over-parameterized networks and Theorem \ref{thm:lower_bound_specific} for networks with $k=2$. We formally show this in \secref{sec:cor_proof}. In \secref{sec:overparam} we state Theorem \ref{thm:main} and outline its proof. In \secref{sec:k2} we state Theorem \ref{thm:lower_bound_specific} and shortly outline its proof. Finally, for completeness, in \secref{sec:xor} we also provide a convergence guarantee for the XOR problem  with inputs in $\{\pm1\}$, which in our setting is the case of $d=1$. In what follows, we will need the following formal definition for a detection of a pattern by a network. 
% For completeness we also include in this section an optimization guarantee for the XOR problem defined in the introduction (Theorem \ref{thm:xor})
\begin{definition}
\label{def:detection}
Let $c_d \ge 0$ be a constant. For each positive pattern $\vv_p$ define $D_{\vv_p} = \sum_{i=1}^k{\sigma\left(\wvec{i}\cdot \vv_p\right)}$ and for each negative pattern $\vv_n$ define $D_{\vv_n} = \sum_{i=1}^k{\sigma\left(\uvec{i}\cdot \vv_n\right)}$. We say that a pattern $\vv$ (positive or negative) is detected by the network $\net$ with confidence $c_d$ if $D_{\vv} > c_d$.
\end{definition}


The above definition captures a desired property of a network, namely, that its filters which are connected with a positive coefficient in the last layer, have high correlation with the positive patterns and analogously for the remaining filters and negative patterns. We note however, that the condition in which a network detects all patterns is not equivalent to realizing the ground truth $f^*$. The former can hold without the latter and vice versa.

 Theorem \ref{thm:main} and Theorem \ref{thm:lower_bound_specific} together imply a clear characterization of the different inductive biases of gradient descent in the case of small ($k=2$) and over-parameterized networks. The characterization is that over-parameterized networks are biased towards global minima that detect all patterns in the data, whereas small networks with $k=2$ are biased towards global minima that do not detect all patterns (see Definition \ref{def:detection}). In \secref{sec:exp_patterns} we show this empirically in the XORD problem and in a generalization of the XORD problem.

In the following sections we will need several notations. Define $\xx_1=(1,1),  \xx_2=(1,-1), \xx_3=(-1,-1), \xx_4=(-1,1)$ to be the four possible patterns in the data and the following sets:
\begin{align*}
\label{eq:sets}
W_t^+(i) = \left\{j \mid \argmax_{1 \le l \le 4} \wvec{j}_t\cdot \xx_l = i \right\},\,\,U_t^+(i) = \left\{j \mid \argmax_{1 \le l \le 4} \uvec{j}_t\cdot \xx_l = i \right\} \\
W_t^-(i) = \left\{j \mid \argmax_{l \in \{2,4\}} \wvec{j}_t\cdot \xx_l = i \right\},\,\,U_t^-(i) = \left\{j \mid \argmax_{l \in \{2,4\}} \uvec{j}_t\cdot \xx_l = i \right\} \numberthis
\end{align*}



We denote by $\xx^+$ a positive diverse point and $\xx^-$ a negative diverse point. Define the following sum:
$$S_t^+ = \sum_{j \in W_t^+(1) \cup W_t^+(3)}\left[\max\left\{\sigma\left(\wvec{j}\cdot \xx_1^+ \right),...,\sigma\left(\wvec{j}\cdot \xx_d^+ \right)\right\}\right]$$
Finally, in all of the results in this section we will denote by $c < 10^{-10}$ a negligible constant.

\subsection{Sample Complexity Upper Bound for Over-parameterized Networks}
\label{sec:overparam} 

The main result in this section is given by the following theorem.
\begin{thm}
	\label{thm:main}
	Let $S=S_+\cup S_-$ be a training set as in \secref{sec:xord_problem_formulation}. Assume that gradient descent runs with parameters $\eta = \frac{\ceta}{k}$ where $\ceta \le \frac{1}{410}$, $\sigma_g \le \frac{\ceta}{16k^{\frac{3}{2}}}$, $k \ge 120$ and $\gamma \ge 8$. Then, with probability at least $\left(p_+p_-\right)^m\left(1-c - 16e^{-8}\right)$ after running gradient descent for $T \ge \frac{28(\gamma + 1 + 8\ceta)}{\ceta}$ iterations, it converges to a global minimum which satisfies:
	\begin{enumerate}
		\item $\sign\left(\nett{T}(\xx)\right) = f^*(\xx)$ for all $\xx \in \{\pm1\}^{2d}$.
		\item Let $\alpha(k) = \frac{\frac{k}{4}+2\sqrt{k}}{\frac{k}{4}-2\sqrt{k}}$. Then for $c_d \le \frac{1 - \frac{5\ceta}{4}}{\alpha(k)+1}$, all patterns are detected with confidence $c_d$.
	\end{enumerate}
\end{thm}

This result shows that given a small training set size, and sufficiently large $p_+$ and $p_-$, over-parameterized networks converge to a global minimum which realizes the classifier $f^*$ with high probability and in a constant number of iterations. Furthermore, this global minimum detects all patterns in the data with confidence that increases with over-parameterization. The full proof of Theorem \ref{thm:main} is given in \secref{sec:proof_overparam}. 

We will now sketch its proof. With probability at least $\left(p_+p_-\right)^m$ all training points are diverse and we will condition on this event. From \secref{sec:vc} we can assume WLOG that the training set consists of one positive diverse point $\xx^+$ and one negative diverse point $\xx^-$ (since the network will have the same output on all same-label diverse points). 
We note that empirically over-parameterization improves generalization even when the training set contains non-diverse points (see \figref{fig:xor_over_param} and \secref{sec:exp_setups}).
% shows this is the case. See \secref{sec:exp_setups} for further details. 
%We leave the analysis of this case for future work.

Now, to understand the dynamics of gradient descent it is crucial to understand the dynamics of the sets in \eqref{eq:sets}. This follows since the gradient updates are expressed via these sets. Concretely, let $j \in W_t^+(i_1)\cap W_t^-(i_2)$ then the gradient update is given as follows: \footnote{Note that with probability 1, $\sigma'(\wvec{j}_t\cdot\xx_{i_1})=1$, $\sigma'(\wvec{j}_t\cdot\xx_{i_2})=1$ for all $t$, and therefore we omit these from the gradient update. This follows since $\sigma'(\wvec{j}_t\cdot\xx_{i_1})=0$ for some $t$ only if $\wvec{j}_0\cdot\xx_{i_1}$ is an integer multiple of $\eta$.}
\begin{equation}
\label{eq:w_gradient_sketch}
\wvec{j}_{t+1} = \wvec{j}_{t} + \eta \xx_{i_1}\mathbbm{1}_{\net(\xx^+) < \gamma} - \eta \xx_{i_2}\mathbbm{1}_{\net(\xx^-) < 1}
\end{equation}
Similarly, for $j \in U_t^+(i_1)\cap U_t^-(i_2)$ the gradient update is given by:
\begin{equation}
\label{eq:u_gradient_sketch}
\uvec{j}_{t+1} = \uvec{j}_{t} - \eta \xx_{i_1}\mathbbm{1}_{\net(\xx^+) < \gamma} + \eta \xx_{i_2}\mathbbm{1}_{\net(\xx^-) < 1}
\end{equation}
Furthermore, the values of $\net(\xx^+)$ and $\net(\xx^-)$ depend on these sets and their corresponding weight vectors, via sums of the form $S_t^+$, defined above.

The proof consists of a careful analysis of the dynamics of the sets in \eqref{eq:sets} and their corresponding weight vectors. For example, one result of this analysis is that for all $t \ge 1$ and $i \in \{1,3\}$ we have $W_t^+(i) = W_0^+(i)$ and the size of $W_t^+(i)$ is at least $\frac{k}{2} - 2\sqrt{k}$ with high probability. 
 
There are two key technical observations that we apply in this analysis. First, with a small initialization and with high probability, for all $1 \le j \le k $ and $1 \le i \le 4$ it holds that $\abs{\wvec{j}_0 \cdot \xx_i} \le \frac{\eta}{4}$ and $\abs{\uvec{j}_0 \cdot \xx_i} \le \frac{\eta}{4}$. This allows us to keep track of the dynamics of the sets in \eqref{eq:sets} more easily. For example, by this observation it follows that if for some $j^* \in W_t^+(2)$ it holds that $j^* \in W_{t+1}^+(4)$, then \textit{for all} $j$ such that $j \in W_t^+(2)$ it holds that $j \in W_{t+1}^+(4)$. Hence, we can reason about the dynamics of several filters all at once, instead of each one separately. Second, by concentration of measure we can estimate the sizes of the sets in \eqref{eq:sets} at iteration $t=0$. Combining this with results of the kind $W_t^+(i) = W_0^+(i)$ for all $t$, we can understand the dynamics of these sets throughout the optimization process.

The theorem consists of optimization and generalization guarantees. For the optimization guarantee we show that gradient descent converges to a global minimum. To show this, the idea is to characterize the dynamics of $S_t^+$ using the characterization of the sets in \eqref{eq:sets} and their corresponding weight vectors. We show that as long as gradient descent did not converge to a global minimum, $S_t^+$ cannot decrease in any iteration and it is upper bounded by a constant. Furthermore, we show that there cannot be too many consecutive iterations in which $S_t^+$ does not increase. Therefore, after sufficiently many iterations gradient descent will converge to a global minimum.


We will now outline the proof of the generalization guarantee. Denote the network learned by gradient descent by $\nett{T}$. First, we show that the network classifies all positive points correctly.
Define the following sums for all $1 \le i \le 4$:
\be
X^+_t(i) = \sum_{j \in W_T^+(i)}\max_k \sigma\left(\wvec{j}\cdot \xx_k^+ \right) \ \ , \ \ 
Y^+_t(i) = \sum_{j \in U_T^+(i)}\max_k\sigma\left(\uvec{j}\cdot \xx_k^+ \right)
\ee

First we notice that for all positive $\zz$ we have $\nett{T}(\zz) \gtrapprox  \min\{X_T^+(1),X_T^+(3)\} - Y_T^+(2) - Y_T^+(4)$.
Then by the fact that $\nett{T}(\xx^+) \ge \gamma$ at the global minimum, we can show that $X_T^+(1) + X_T^+(3)$ is sufficiently large. As mentioned previously, by concentration of measure, $\abs{W_0^+(i)}$ is sufficiently large. Then by a symmetry argument we show that this implies that both $X_T^+(1)$ and $X_T^+(3)$ are sufficiently large. This shows that patterns $\xx_1$ and $\xx_3$ are detected. Finally, we show that $Y_T^+(2) + Y_T^+(4)$ is not too large due to an upper bound on $-\nett{T}(\xx^-)$. Hence, we can show that each positive point is classified correctly. The proof that all negative points are classified correctly and patterns $\xx_2$ and $\xx_4$ are detected is similar but slightly more technical. We refer the reader to \secref{sec:proof_overparam} for further details.


\ignore{
Finally, for completeness, we prove the following convergence guarantee for the XOR problem, where $d = 1$. Note that in the case of two dimensions, the convolutional network introduced in \secref{sec:problem_formulation} reduces to a two-layer fully connected network. The analysis is similar to the analysis of Theorem \ref{thm:main}, but considerably simpler. The proof is given in \secref{sec:xor}.

\begin{thm}
	\label{thm:xor}
	Consider the training set $S=\{(\xx_1,1),(\xx_2,-1),(\xx_3,1),(\xx_4,-1)\}$, where $\xx_1 = (1,1)$, $\xx_2 = (-1,1)$, $\xx_3 = (-1,-1)$ and $\xx_4 = (1,-1)$. Assume that gradient descent runs with parameters $\eta = \frac{\ceta}{k}$ where $\ceta \le 1$, $\sigma_g \le \frac{\ceta}{16k^{\frac{3}{2}}}$, $k \ge 25$ and $\gamma = 1$. Then, with probability at least $1 - c - 8e^{-8}$, after at most $\frac{4k}{k-2\sqrt{k}} + 40$ iterations, gradient descent converges to a global minimum.
\end{thm}
}

\subsection{Sample Complexity Lower Bound for Small Networks ($k=2$)}
\label{sec:k2}

The following theorem provides generalization lower bounds of global minima in the case that $k=2$ and in a slightly more general setting than the one given in Theorem \ref{thm:main}.

\begin{thm}
	\label{thm:lower_bound_specific}
	Let $S=S_+\cup S_-$ be a training set as in \secref{sec:problem_formulation}. Assume that gradient descent runs with parameters $\eta = \frac{\ceta}{k}$ where $\ceta \le \frac{1}{41}$, $\sigma_g \le \frac{\ceta}{16k^{\frac{3}{2}}}$, $k = 2$ and $\gamma \ge 1$.
	Then the following holds:
	\begin{enumerate}
		\item With probability at least $\left(p_+p_-\right)^m\left(1-c\right)\frac{33}{48}$, gradient descent converges to a global minimum that has non-zero test error. Furthermore, for $c_d \ge 2\ceta$, there exists at least one pattern which is not detected by the global minimum with confidence $c_d$. 
		\item The non-zero test error above is at least $p^*$.
	\end{enumerate}	
\end{thm}

%\item Let $M > 0$ and $T$ be an iteration which is the minimum between $M$ and the first iteration which gradient descent converges to a global minimum. \footnote{The definition of iteration $T$ can be thought as a stopping rule - if gradient descent did not converge to a global minimum until iteration $M$, then stop it.}Then, with probability at least $\left(1-\delta\right)\left(1-\sqrt{\frac{8}{\pi}}e^{-32}\right)\frac{15}{16}$, the network at iteration $T$ has non-zero test error, i.e., there exists $\xx \in \{\pm1\}^{2d}$ such that  $\sign\left(\nett{T}(\xx)\right) \neq f^*(\xx)$. 

The theorem shows that for a training set that is not too large and given sufficiently large $p_+$ and $p_-$, with constant probability, gradient descent will converge to a global minimum that is not the classifier $f^*$. Furthermore, this global minimum does not detect at least one pattern. The proof of the theorem is given in \secref{sec:proof_lower_bound}.

We will now provide a short outline of the proof. Let $\wvec{1}_T$, $\wvec{2}_T$, $\uvec{1}_T$ and $\uvec{2}_T$ be the filters of the network at the iteration $T$ in which gradient descent converges to a global minimum. The proof shows that gradient descent will not learn $f^*$ if one of the following conditions is met: a) $W_T^+(1) = \emptyset$. b) $W_T^+(3) = \emptyset$. c) $\uvec{1}_T \cdot \xx_2 > 0$ and $\uvec{2}_T \cdot \xx_2 > 0$. d) $\uvec{1}_T \cdot \xx_4 > 0$ and $\uvec{2}_T \cdot \xx_4 > 0$.
%\begin{enumerate}
%	\label{en:event_E}
%	\item $W_T^+(1) = \emptyset$.
%	\item $W_T^+(3) = \emptyset$.
%	\item $\uvec{1} \cdot \xx_2 > 0$ and $\uvec{2} \cdot \xx_2 > 0$.
%	\item $\uvec{1} \cdot \xx_4 > 0$ and $\uvec{2} \cdot \xx_4 > 0$.
%\end{enumerate}
Then by using a symmetry argument which is based on the symmetry of the initialization and the training data it can be shown that one of the above conditions is met with high constant probability. Finally, it can be shown that if one of these conditions hold, then at least one pattern is not detected.


%Finally, we note that there is a clear connection between detection of all patterns and the ability of a network to realize $f^*$. Namely, that for sufficiently small $c_d$, the condition that the network detects all patterns in the data is necessary but not sufficient for the network to realize the function $f^*$. To show this connection, first note that if all the patterns are detected by a network $\net$ and for all positive patterns $\vv_p$ and negative patterns $\vv_n$ it holds that $D_{\vv_p} >> D_{\vv_n}$ and $D_{\vv_p}$ and $D_{\vv_p}$ are both sufficiently large, then the network will realize the function $f^*$. If it only holds that all patterns are detected, then it may be the case that the network does not realize $f^*$, e.g., when $D_{\vv_p} << D_{\vv_n}$ for some positive pattern $\vv_p$ and negative pattern $\vv_n$. Furthermore, for sufficiently small $c$, if only a fraction of the patterns are detected, the network will not realize $f^*$. For example, if the network detected some of the negative patterns but not all of the positive patterns, then there will be positive points that it will not classify correctly. The other cases follow similarly.




